Centrality evolution of the charged-particle pseudorapidity density over a broad pseudorapidity range in Pb-Pb collisions at $\sqrt{s_{\rm NN}}$ = 2.76 TeV

The centrality dependence of the charged-particle pseudorapidity density measured with ALICE in Pb-Pb collisions at $\sqrt{s_{\rm NN}}$ over a broad pseudorapidity range is presented. This Letter extends the previous results reported by ALICE to more peripheral collisions. No strong change of the charged-particle pseudorapidity density distributions with centrality is observed, and when normalised to the number of participating nucleons in the collisions, the evolution over pseudorapidity with centrality is likewise small. The broad pseudorapidity range allows precise estimates of the total number of produced charged particles which we find to range from $162\pm22$ (syst.) to $17170\pm770$ (syst.) in 80-90% and 0-5 central collisions, respectively. The total charged-particle multiplicity is seen to approximately scale with the number of participating nucleons in the collision. This suggests that hard contributions to the charged-particle multiplicity are limited. The results are compared to models which describe $\mbox{d}N_{\mbox{ch}}/\mbox{d}\eta$ at mid-rapidity in the most central Pb-Pb collisions and it is found that these models do not capture all features of the distributions.

==> texs/notes.tex <==
\section{Notes for the IRC \textit{et al}}
\subsection*{8/8-'15}
\begin{itemize}
\item Implemented Lee's comments
\item Implemented most of Domenicos comments. 
\item Took out MC quantitative comparison --- sigh, back to ``as can
  [clearly] be seen''
\end{itemize}

\subsection*{5/8-'15}
\begin{itemize}
\item Implemented most comments from the 3/9-'15 IRC review. 
\item Changed order of \figref{fig:fitsnpart} and \ref{fig:nparteta},
  and the corresponding text.  In the abstract, introduction, and
  conclusion, the $\ndndeta$ versus $N_{\text{part}}$ comes before
  $N_{\text{total}}$ 
\item With the help of Lee, we've tried to make the abstract,
  introduction, and conclusion more `crispy' --- that is, being
  pertinent, concise, and interesting. 
\item It was decided to keep the Kolomogorov--Smirnov test in and try
  it out with the collaboration.  If there's strong objections, we
  will take it out. 
\item I do not have a good reference for \texttt{AliGenTunedOnPbPb},
  so if someone has that, please let me know. 
\item Fixed the \textsf{hyperref} {\color{alicered}
    co}{\color{aliceyellow} lo}{\color{alicepurple} ur}s so the text
  is easier to read without annoying boxes.
\end{itemize}


\subsection*{28/7-'15} 
\begin{itemize}
\item `Optimized' figures for CERN pre-print style
\item Sigh --- yet another small error in the calculation of the
  $\chi^2/\nu$ (forgot to square errors on \centRange{0}{30} points). 
\item Added Kolomogorov--Smirnov test. 
\item Made MC comparisons a $2\times4$ plot with option for
  $2\times3$. 
\item Added some words motivating the fit functions for extracting
  $N_{total}$ 
\item Explained a bit more how cuts where varied and obtained. 
\item Highlight difference between AMPT with and without string
  melting. 
\item Fixed a few language issues. 
\end{itemize}

\ifmcquant
\begin{figure}[htbp]
  \centering
\ifmcchi
  \figinput{ModelKS}
  \caption{[NOT FOR THE PAPER] Kolomogorov test}
\else 
  \figinput{ModelChi2}
  \caption{[NOT FOR THE PAPER] $\chi^{2}/\nu$ test}
\fi
  \label{fig:app:quant}
\end{figure}
\else
\begin{figure}[htbp]
  \centering
  \figinput{ModelKS}
  \figinput{ModelChi2}
  \caption{[NOT FOR THE PAPER] Kolomogorov test and $\chi^{2}/\nu$ test}
  \label{fig:app:quant}
  \label{fig:modelchi2}
\end{figure}
\fi


\begin{figure}[htbp]
  \centering
  \figinput{Models6}
  \caption{[NOT FOR THE PAPER] MC comparison $2\times3$}
  \label{fig:app:mc}
\end{figure}


\subsection*{21/7-'15}
\begin{itemize}
\item Data in \figref{fig:modelchi2} was wrongly calculated in last
  draft.  Corrected here. 
\item Now use CERN pre-print style
\item Use EPS
\item Merged in comments from Alberica, Lee, Ruben, and Marek
\item Added AMPT w/string melting to \figref{fig:Models}
\item Added \figref{fig:nparteta}
\item Added phobos to \figref{fig:fitsnpart}
\item Added Bjorken--inspired function \eqref{eq:bjorken} 
\item Added missing references etc. 
\end{itemize}

\subsection*{7/7-'15}
\begin{itemize}
\item Language is British-English. 
\item Plain \LaTeX{} with a few `standard' packages (no CERN specific
  styles or Bib\TeX{} styles)
\item This draft (7\textsuperscript{th} of July, 2015) is intended to
  help us discuss content.  Wording, language, style, etc. comments
  are welcome but should be secondary.  
\item Some references are missing here and there. I've tried to mark
  them 
\item `Fixme's are shown with {\color{alicered} red} number in the
  margin, and corresponding {\color{alicered} red} footnotes. 
\item The source lives in the EB Subversion repository:\\
  \texttt{https://svnweb.cern.ch/cern/wsvn/alipap/id1613/}
\end{itemize}

%% Local Variables:
%%  TeX-master: "../cds"
%%  ispell-local-dictionary: "british"
%% End:

%  LocalWords:  tracklets scintillator tracklet centralities
%  LocalWords:  symmetrised

